Heterogeneity-Guided Client Sampling: Towards Fast and Efficient Non-IID Federated Learning

Statistical heterogeneity of data present at client devices in a federated learning (FL) system renders the training of a global model in such systems difficult. Particularly challenging are the settings where due to communication resource constraints only a small fraction of clients can participate in any given round of FL. Recent approaches to training a global model in FL systems with non-IID data have focused on developing client selection methods that aim to sample clients with more informative updates of the model. However, existing client selection techniques either introduce significant computation overhead or perform well only in the scenarios where clients have data with similar heterogeneity profiles. In this paper, we propose HiCS-FL (Federated Learning via Hierarchical Clustered Sampling), a novel client selection method in which the server estimates statistical heterogeneity of a client's data using the client's update of the network's output layer and relies on this information to cluster and sample the clients. We analyze the ability of the proposed techniques to compare heterogeneity of different datasets, and characterize convergence of the training process that deploys the introduced client selection method. Extensive experimental results demonstrate that in non-IID settings HiCS-FL achieves faster convergence than state-of-the-art FL client selection schemes. Notably, HiCS-FL drastically reduces computation cost compared to existing selection schemes and is adaptable to different heterogeneity scenarios.

==> src/table1r.tex <==
\begin{table*}[!h]
\caption{A comparison between HiCS and its variant (denoted "Oracle") obtained by replacing $\hat{H}(\mathcal{D}^{(k)})$ in Eq.9 by the true entropy. All other settings remain intact. $\text{ACC}_{T}$ (\%) denotes the test accuracy after $T$ global rounds and $t_{\text{acc}}$ denotes the required number of rounds to achieve target accuracy $acc$. }
\vspace{-0.1 in}
\scriptsize
\begin{center}
\label{table1r}
\begin{tabular}{ccccccccc}
\bottomrule[1pt]
\multirow{2}{*}{Setting} & \multicolumn{2}{c}{CIFAR10 (1)}  &\multicolumn{2}{c}{CIFAR10 (2)} & \multicolumn{2}{c}{Mini (1)} & \multicolumn{2}{c}{Mini (2)} \\
\cline{2-9}
  & $\text{ACC}_{500}$ & $t_{65\%}$ & $\text{ACC}_{500}$ & $t_{65\%}$  & $\text{ACC}_{100}$ & $t_{50\%}$  & $\text{ACC}_{100}$ & $t_{50\%}$ \\
\hline
HiCS-FL     
 &  65.5 & 377 &  60.1 & 123  &  50.5 & 52 &51.2 & 86
  \\
Oracle  &\textbf{ 68.6}& \textbf{231} & \textbf{63.8}& \textbf{99} &\textbf{52.2}  & \textbf{45}&\textbf{53.1} & \textbf{40} \\

\toprule[1pt]
\end{tabular}
\end{center}
\vspace{-0.15in}
\end{table*}

==> src/table2r.tex <==
\begin{table*}[!h]
\caption{The results (accuracy in \%) of experiments with varied values of $\lambda$ (CS denotes Clustered Sampling). "FM" denotes FMNIST; "C10" denotes CIFAR10 and "Mini" denotes Mini-ImageNet. }
\vspace{-0.1 in}
\scriptsize
\begin{center}
\label{table2r}
\begin{tabular}{ccccccccc}
\bottomrule[1pt]
$\lambda$ & FM (1) & FM (2)&FM (3) & C10 (1) & C10 (2)&C10 (3) & Mini (1) & Mini(2)\\
\hline
CS ($\lambda$ = 0)    
 &  80.1 & 75.6 &  67.5 & 60.4  &  49.1 & 39.0 & 46.7& 47.4
  \\
1  &83.8 & 78.5 & 68.1 &62.1 &56.2 &40.4 &49.2 &48.1  \\
5  &87.4 &80.0 & 68.9 & 62.7& 57.3 & 47.7&49.5 &48.1 \\
10  &\textbf{87.6} &\textbf{81.5} &\textbf{69.6} &\textbf{65.5} &59.8 &\textbf{50.6} &\textbf{50.5} &\textbf{51.2}\\
20  &87.0 &76.4 &68.5 &62.1 &\textbf{60.4} &49.2 &49.5 &50.4 \\
\toprule[1pt]
\end{tabular}
\end{center}
\vspace{-0.15in}
\end{table*}

==> src/table3r.tex <==
\begin{table*}[!h]
\caption{The results (accuracy in \%) of inference tests on the local data from the same distribution as in fine-tuning. All the settings are as described in the paper. }
\vspace{-0.1 in}
\scriptsize
\begin{center}
\label{table3r}
\begin{tabular}{ccccccc}
\bottomrule[1pt]
Scheme & Random & pow-d&DivFL & CS &FedCor &HiCS-FL\\
\hline
CIFAR10 (1)   
 &  85.6 & 86.7 & 84.0 & 86.2 & 80.8 &\textbf{87.4}\\
CIFAR10 (2)  &93.7 & 93.3 & 91.6 & 93.7 & 93.7 &\textbf{94.7}\\
CIFAR10 (3)  &94.5 & 94.7 &93.9 &94.5& 95.0 & \textbf{95.8}\\
Mini-ImageNet (1)  &67.3 & 67.2 &67.5 &67.8 &68.7 &\textbf{69.0} \\
Mini-ImageNet (2)  & 71.2 &71.8 &72.1 &72.1 &\textbf{72.7 }& 72.5\\
\toprule[1pt]
\end{tabular}
\end{center}
\vspace{-0.15in}
\end{table*}

==> src/table4r.tex <==
\begin{table*}[!h]
\caption{A comparison between HiCS and Oort. Experimental settings as same as those used to generate results in Table \ref{table1r}. $\text{ACC}_{T}$ (\%) denotes the test accuracy after $T$ global rounds and $t_{acc}$ denotes the required number of rounds to achieve target accuracy $acc$. "-" denotes the method can not converge to target accuracy.}
\vspace{-0.1 in}
\scriptsize
\begin{center}
\label{table4r}
\begin{tabular}{ccccccccc}
\bottomrule[1pt]
\multirow{2}{*}{Setting} & \multicolumn{2}{c}{FMNIST (1)}  &\multicolumn{2}{c}{FMNIST (2)} & \multicolumn{2}{c}{FMNIST (3)} & \multicolumn{2}{c}{Mini (1)} \\
\cline{2-9}
  & $\text{ACC}_{200}$ & $t_{85\%}$ & $\text{ACC}_{200}$ & $t_{75\%}$  & $\text{ACC}_{200}$ & $t_{65\%}$  & $\text{ACC}_{100}$ & $t_{50\%}$ \\
\hline
HiCS-FL     
 & \textbf{87.6} &\textbf{30} & \textbf{81.5} &\textbf{60} &\textbf{69.6} &\textbf{67} &\textbf{50.5} &\textbf{52}
  \\
Oort  &86.2 & 94 &75.9 &109 & 56.8 & - &50.4 &84\\
\hline
\multirow{2}{*}{Setting} & \multicolumn{2}{c}{CIFAR10 (1)}  &\multicolumn{2}{c}{CIFAR10 (2)} & \multicolumn{2}{c}{CIFAR10 (3)} & \multicolumn{2}{c}{Mini (2)} \\
\cline{2-9}
  & $\text{ACC}_{500}$ & $t_{65\%}$ & $\text{ACC}_{500}$ & $t_{60\%}$  & $\text{ACC}_{500}$ & $t_{50\%}$  & $\text{ACC}_{100}$ & $t_{50\%}$ \\
\hline
HiCS-FL     
 &  \textbf{65.5} &\textbf{377} &\textbf{60.1} &\textbf{123} &50.6 &\textbf{149} &\textbf{51.2} &\textbf{86}
  \\
Oort  &65.3 &399 &59.8 &299 &\textbf{50.9} &400 &48.2 &127\\
\toprule[1pt]
\end{tabular}
\end{center}
\end{table*}

==> src/table5r.tex <==
\begin{table*}[!h]
\caption{Additional experimental results (accuracy in \%) on HiCS with the number of clusters $M \leq K$, where $K$ is the number of selected clients each global round. }
\vspace{-0.1 in}
\scriptsize
\begin{center}
\label{table2r}
\begin{tabular}{cccccc}
\bottomrule[1pt]
$M$ & CIFAR10 (1) & CIFAR10 (2)&CIFAR10 (3) & Mini (1) & Mini(2)\\
\hline
$M = 0.3K$  
 & 61.3 &57.0 &47.5 &50.4 &50.1
  \\
$M = 0.5K$  &65.1 &\textbf{61.5} &46.2 &49.8 &50.4 \\
$M = 0.7K$  &62.8 &59.2 &\textbf{51.2} &\textbf{51.1} &49.9\\
$M = K$ &\textbf{65.5} & 59.8 &50.6 &50.5 &\textbf{51.2}\\
\toprule[1pt]
\end{tabular}
\end{center}
\vspace{-0.15in}
\end{table*}

==> src/table6r.tex <==
\begin{table*}[!h]
\caption{In experiments on CIFAR10, only 20 out of 50 clients are available in the beginning; additional 10 clients join each 100 global rounds. The initial 20 clients leave the system after 400 global rounds. }
\vspace{-0.1 in}
\scriptsize
\begin{center}
\label{table6r}
\begin{tabular}{ccccccc}
\bottomrule[1pt]
Scheme & Random & pow-d&DivFL & CS &FedCor &HiCS-FL\\
\hline
CIFAR10 (1)   
 &  85.6 & 86.7 & 84.0 & 86.2 & 80.8 &\textbf{87.4}\\
CIFAR10 (2)  &93.7 & 93.3 & 91.6 & 93.7 & 93.7 &\textbf{94.7}\\
CIFAR10 (3)  &94.5 & 94.7 &93.9 &94.5& 95.0 & \textbf{95.8}\\
Mini-ImageNet (1)  &67.3 & 67.2 &67.5 &67.8 &68.7 &\textbf{69.0} \\
Mini-ImageNet (2)  & 71.2 &71.8 &72.1 &72.1 &\textbf{72.7 }& 72.5\\
\toprule[1pt]
\end{tabular}
\end{center}
\vspace{-0.15in}
\end{table*}
